First measurement of transverse-spin-dependent azimuthal asymmetries in the Drell-Yan process

The first measurement of transverse-spin-dependent azimuthal asymmetries in the pion-induced Drell-Yan (DY) process is reported. We use the CERN SPS 190 GeV/$c$, $\pi^{-}$ beam and a transversely polarized ammonia target. Three azimuthal asymmetries giving access to different transverse-momentum-dependent (TMD) parton distribution functions (PDFs) are extracted using dimuon events with invariant mass between 4.3 GeV/$c^2$ and 8.5 GeV/$c^2$. The observed sign of the Sivers asymmetry is found to be consistent with the fundamental prediction of Quantum Chromodynamics (QCD) that the Sivers TMD PDFs extracted from DY have a sign opposite to the one extracted from semi-inclusive deep-inelastic scattering (SIDIS) data. We present two other asymmetries originating from the pion Boer-Mulders TMD PDFs convoluted with either the nucleon transversity or pretzelosity TMD PDFs. These DY results are obtained at a hard scale comparable to that of a recent COMPASS SIDIS measurement and hence allow unique tests of fundamental QCD universality predictions.

==> acknowledge.tex <==
We gratefully acknowledge the support of the CERN management and staff 
and the skill and effort of the technicians of our collaborating institutes.

This work was made possible by the financial support of our funding agencies:
MEYS (Czech Republic) Grant LG13031; 
FP7 ``HadronPhysics3'' Grant 283286 (European Union); 
CEA, P2I and ANR (France); 
BMBF, DFG cluster of excellence ``Origin and Structure of the Universe'',
DFG Research Training Group Programmes 1102 and 2044 (Germany); 
B.Sen fund (India); 
Academy of Sciences and Humanities (Israel); 
INFN (Italy); 
MEXT and JSPS, Grants 8002006, 20540299 and 18540281, Daiko and Yamada Foundations (Japan); 
NCN Grant 2015/18/M/ST2/00550 (Poland); 
FCT COMPETE and QREN, Grants CERN/FP 116376/2010, 123600/2011 and CERN/FIS-NUC/0017/2015 (Portugal); 
CERN-RFBR Grant 12-02-91500, Presidential Grant NSh-999.2014.2 (Russia);
MST (Taiwan)and
NSF (USA).


